Lateral-Direction Localization Attack in High-Level Autonomous Driving: Domain-Specific Defense Opportunity via Lane Detection

Localization in high-level Autonomous Driving (AD) systems is highly security critical. While the popular Multi-Sensor Fusion (MSF) based design can be more robust against single-source sensor spoofing attacks, it is found recently that state-of-the-art MSF algorithms is vulnerable to GPS spoofing alone due to practical factors, which can cause various road hazards such as driving off road or onto the wrong way. In this work, we perform the first systematic exploration of the novel usage of lane detection (LD) to defend against such attacks. We first systematically analyze the potentials of such a domain-specific defense opportunity, and then design a novel LD-based defense approach, $LD^3$, that aims at not only detecting such attacks effectively in the real time, but also safely stopping the victim in the ego lane upon detection considering the absence of onboard human drivers. We evaluate $LD^3$ on real-world sensor traces and find that it can achieve effective and timely detection against existing attack with 100% true positive rates and 0% false positive rates. Results also show that $LD^3$ is robust to diverse environmental conditions and is effective at steering the AD vehicle to safely stop within the current traffic lane. We implement $LD^3$ on two open-source high-level AD systems, Baidu Apollo and Autoware, and validate its defense capability in both simulation and the physical world in end-to-end driving. We further conduct adaptive attack evaluations and find that $LD^3$ is effective at bounding the deviations from reaching the attack goals in stealthy attacks and is robust to latest LD-side attack.

==> discovery.tex <==
\nsection{Lane Boundary: Defense-Suitable Information Source for High-Level AD Localization} \label{sec:discovery}
% \nsection{Lane Detection: Defense-Suitable Information Source for High-Level AD Localization} \label{sec:discovery}

% Since defenses for high-level AD systems have the freedom to leverage other information sources, we aim to address \textbf{C1} by identifying the ones that are suitable for defending against lateral direction localization attacks.
% As mentioned in~\S\ref{sec:motivation_challenges}, such information sources may never provide more accurate positioning than the existing ones used in AD localization in common circumstances, however, they may be useful for defense purposes when the AD localization is substantially wrong due to attacks.
% More concretely, we need to find the ones that are

% Specifically, such sources should be ``\textit{defense-suitable}'' for high-level AD localization, i.e., they should be (1) \textit{independent of the ones that are already used for AD localization}, and (2) \textit{reliable when the sources are applicable}. Otherwise, attacks targeting these information sources may break the defense and AD localization at the same time and lead to false negatives, or the defense may have high false positives in benign drivings.

% Moreover, it is also challenging to leverage the information source for detection purpose if it does not directly measure the vehicle's global position.
% such that the defense does not introduce false positives when the information source is applicable.
% reasonable in security since the attacker wants to make the systems substantially wrong
% Limited scope: Longitudinal direction is not suitable for localization accuracy
% Not considered for AD developers since they emphasize on the accuracy
% In the cases when the data is applicable, the information is accurate
% Lateral direction
% To address this, leverage other sources, requirements: independent, reliable (not much FP) (define what is defense-suitable, e.g., what are the requirements); but challenging: if a sensor is useful for localization, should already be used → must be some limitations with those sources → defense is more important than accuracy → could be used for cross checking; repurpose the sensor for our defense purpose

To address \textbf{C1}, a natural information source directly related to lateral-direction attacks is the relative distance to the current lane boundaries, which is generally available during driving and also can be obtained via mature technologies such as camera-based lane detection~\cite{hillel2014recent, openpilot, pan2018spatial}. However, we find that state-of-the-art AD localization algorithms actually do not use such features~\cite{wan2018robust, autoware, gao2015ins, soloviev2008tight, udacity_av_apollo, udacity_av_nd, coursera_av}, as they can only tell \textit{local} lateral positions specific to the current lane; for the purpose of \textit{global} localization on the map in the world coordinate system needed by high-level AD systems, they are almost useless as they are not generally distinctive across different roads and regions.
% on the map.

% Although not of much use from the functionality perspective, we find that it does qualify as a defense-suitable information source for AD localization, e.g., independence to existing sources/features used in state-of-the-art algorithms and reliability when applicable.

As mentioned in \S\ref{sec:motivation_challenges}, defense-suitable sources need to satisfy the independence and reliability requirements. 
Since lane detection techniques are already very mature~\cite{hillel2014recent}, thus they are presumably reliable in practice, which will also be empirically proven in our evaluations later (\S\ref{sec:eval}).
However, it is unclear if lane boundaries are independent of the ones already used in AD localization as LiDAR can also sense the lane line markings. Since LiDAR locator is the only one among the MSF inputs (\S\ref{sec:background_msf_attack}) that is possible to utilize lane boundaries, 
% we thus quantify the relationship between LiDAR locator and the lane boundaries, 
we thus rigorous validate its independence to LiDAR locators.
% via experiments.

% To prove the independence, we aim to find that whether the existing information sources in AD localization use lane boundary information for localization. Among the inputs in MSF localization (\S\ref{sec:background_msf_attack}), LiDAR locator is the only one that is possible to utilize lane boundaries. Intuitively, lane boundaries are ``boring'' features for global localization since they are prevalent on roads and are visually similar when the vehicle is driving. Nevertheless, we still aim to quantify the relationship between LiDAR locator and the lane boundaries.

% , if already used, not satisfy independence requirement. thus, this section, rigorously validate its independence experimentally

% Although not of much use from the functionality perspective, we find that it does qualify as a defense-suitable information source for AD localization, e.g., independence to existing sources/features used in state-of-the-art algorithms and reliability when applicable.


% they are not used for localization purposes in today's high-level AD systems~\cite{apollo, autoware}. However, they appear to be a promising information source for defense purpose since AD localization attacks need to at least achieve lane-straddling lateral deviations to cause real world consequences.


% One such information source available in high-level AD systems is the \textit{lane boundaries}, which can help determine the vehicle the relative position within the current driving lane. They are widely-used for Automated Lane Centering in \textit{lower-level} AD systems, such as openpilot~\cite{openpilot} and Tesla Autopilot~\cite{autopilot}, where \textit{camera-based lane detection} algorithms are applied to identify lane line positions and shapes to help steer the vehicle at the lane center. Since lane boundaries cannot provide accurate global positioning~\cite{kang2020lane, evlampev2020map}, they are not used for localization purposes in today's high-level AD systems~\cite{apollo, autoware}. However, they appear to be a promising information source for defense purpose since AD localization attacks need to at least achieve lane-straddling lateral deviations to cause real world consequences. Thus, we first examine if the lane boundaries information satisfies the independence and reliability requirements as mentioned above. 

% In this section, we focus on evaluating the independence requirement (\S\ref{sec:motivation_challenges}) since lane detection techniques are already very mature~\cite{hillel2014recent} and thus are presumably reliable in practice, which will also be empirically proven in our evaluation later (\S\ref{sec:eval}). To prove the independence, we aim to find that whether the existing information sources in AD localization use lane boundary information for localization. Among the inputs in MSF localization (\S\ref{sec:background_msf_attack}), LiDAR locator is the only one that is possible to utilize lane boundaries. Intuitively, lane boundaries are ``boring'' features for global localization since they are prevalent on roads and are visually similar when the vehicle is driving. Nevertheless, we still aim to quantify the relationship between LiDAR locator and the lane boundaries.


\textbf{Evaluation methodology.} 
To do that, we compare the executions of LiDAR locator with the complete lane boundary information and the one without such information. \textit{If a LiDAR locator does not rely on the lane boundary information, we should observe a high similarity between the two executions.} Specifically, the LiDAR operates by scanning the surrounding environment and outputting point clouds, which store the 3D positions and intensities of the reflected points from the lasers. Lane boundaries, or lane line markings, will exhibit distinctive intensities from the other road surface due to their color differences. Thus, we created the lane line marking removed point cloud data (PCD) by keeping their intensities the same as other road surface area. More technical details on removing the lane line markings is in Appendix~\ref{app:laneline_removal}.

\todo{put correlation analysis using incorrect lane marking information here.}

\textbf{Experimental setup.} 
We evaluate on 2 LiDAR locators, one from Baidu Apollo (BA-LiDAR locator)~\cite{wan2018robust} and another from Autoware (AW-LiDAR locator)~\cite{autoware}. Details of the LiDAR locators can be found in Appendix~\ref{app:lidar_locators}. Since MSF localization takes not only position measurements but also position uncertainties from LiDAR locator as inputs, we calculate both the \textit{position accuracies} and \textit{uncertainty correlation} with and without lane line markings removal to show the similarity.
We evaluated on the same 5 local road and highway traces in \fr{}~\cite{fusionripper} from two datasets. For each trace, we exclude intersections since they do not have lane line markings and thus are out of the applicable domain for lane boundaries. Among them, since \textit{ba-local} does not provide ground truth positions, we calculate the position accuracy based on the LiDAR locator with the complete lane line markings.

% Among them, since \textit{ba-local} does not provide ground truth positions, we calculate the position accuracy based on the LiDAR locator with the complete lane line markings instead of the ground truth positions.

% At design level, Baidu Apollo LiDAR locator (BA-LiDAR locator)~\cite{wan2018robust} considers point cloud intensities in its position calculation. Thus, the removal of lane line intensities do have the potential to affect the BA-LiDAR locator performance. On the other hand, Autoware LiDAR locator (AW-LiDAR locator)~\cite{autoware} only uses the position data in the PCD and completely ignores the intensities. This means that AW-LiDAR locator does not consider lane line markings at the design level. Nevertheless, we still include AW-LiDAR locator in our evaluation. When used in AD localization, the MSF takes not only the position measurement but also the position uncertainty from LiDAR locator as inputs. Thus, we report the \textit{position accuracies} and \textit{uncertainty correlation} with and without lane line markings removal to show the similarity. Specifically, AW-LiDAR locator implements the Normal Distributions Transform (NDT) algorithm~\cite{ndt}, which does not output position uncertainty by default. Thus, we follow a common adaptation for NDT to use the point cloud matching fitness score as the uncertainty~\cite{merten2008three}. We evaluated on the same 5 local road and highway traces in \fr{}~\cite{fusionripper} from two datasets. For each trace, we exclude the road segments that do not have lane line markings, e.g., intersections. Among them, since \textit{ba-local} does not provide ground truth positions, we calculate the position accuracy based on the LiDAR locator with the complete lane line markings instead of the ground truth positions.


\textbf{Results.}
Table~\ref{tbl:correlation} in the Appendix shows the experiment results. For the position accuracy, we report the Root Mean Squared Error (RMSE) between the LiDAR locator positions and the ground truth positions or the ones without lane line marking removal. For the correlation, we use the commonly-used Pearson's correlation, and a correlation coefficient $>$0.5 is considered strongly correlated~\cite{cohen2013statistical}. As shown, the uncertainty correlation coefficients with and without lane line marking removal are all well above the threshold for strong correlation, and their position accuracies are also all at centimeter-level. Particularly, since AW-LiDAR locator does not use lane line markings at the design level (Appendix~\ref{app:lidar_locators}), the traces consequently show perfect correlations and identical position accuracies with and without removing the lane line markings. Such a result suggests that the existing LiDAR locators used in high-level AD systems largely ignore the lane boundary information when localizing the vehicle on the map, which might because global localization focuses more on the unique features on the road, such as buildings, roadside layouts, and traffic signs. As a result, this indicates that lane boundaries are indeed largely independent of the ones that are already used in high-level AD localization and thus pose great potential as a defense-suitable information source.



% \begin{table*}[tbp]
% \footnotesize
% 	\begin{minipage}{0.32\linewidth}
% 		\centering
%         \includegraphics[width=.93\columnwidth]{./figs/lane_line_marking_removal.pdf}
%         \vspace{-0.1in}
%         \captionof{figure}{Demonstration of lane line markings removal. Top figure shows the original PCD; bottom figure shows the one with lane line markings removed.}
%         \label{fig:laneline_removal_example}
% 	\end{minipage}\hfill
% 	\begin{minipage}{0.665\linewidth}
%         \centering
%         \caption{Position uncertainty correlation and position accuracy of LiDAR locators using the original PCDs and lane line markings removed PCDs. For the correlation, we report the Pearson's correlation coefficients. We ignore the $p$-value since they are all statistical significant; the position accuracies are in meters.}
%         \label{tbl:correlation}
%         \setlength{\tabcolsep}{2pt}
%         \begin{tabular}{@{}cccccccc@{}}
%         \toprule
%         \multirow{3}{*}{Trace} & \multicolumn{4}{c}{BA-LiDAR Locator} & \multicolumn{3}{c}{AW-LiDAR Locator} \\ \cmidrule(l){2-8} 
%          & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Uncertainty Correlation\\ (original vs no-marking)\end{tabular}} & \multicolumn{2}{c}{Position Accuracy} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Fitness\\ Correlation\\ (original vs\\ no-marking)\end{tabular}} & \multicolumn{2}{c}{Position Accuracy} \\ \cmidrule(lr){2-5} \cmidrule(l){7-8} 
%          & Easting & Northing & \begin{tabular}[c]{@{}c@{}}RMSE\\ original\end{tabular} & \begin{tabular}[c]{@{}c@{}}RMSE\\ no-marking\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}RMSE\\ original\end{tabular} & \begin{tabular}[c]{@{}c@{}}RMSE\\ no-marking\end{tabular} \\ \midrule
%         ba-local & 0.79 (4e-230) & 0.71 (3e-164) & - & 0.067 & 1.0 (0.0) & - & 0.0 \\
%         ka-local08 & 0.97 (0.0) & 0.98 (0.0) & 0.061 & 0.062 & 1.0 (0.0) & 0.074 & 0.074 \\
%         ka-local31 & 0.98 (0.0) & 0.96 (0.0) & 0.057 & 0.057 & 1.0 (0.0) & 0.077 & 0.077 \\
%         ka-local07 & 0.91 (0.0) & 0.90 (0.0) & 0.077 & 0.080 & 1.0 (0.0) & 0.076 & 0.076 \\
%         ka-highway17 & 0.99 (0.0) & 0.94 (0.0) & 0.059 & 0.060 & 1.0 (0.0) & 0.077 & 0.077 \\
%         ka-highway06 & 0.78 (0.0) & 0.88 (0.0) & 0.064 & 0.064 & 1.0 (0.0) & 0.077 & 0.077 \\ \bottomrule
%         \end{tabular}
% 	\end{minipage}
% \end{table*}

% are represented as $r$ ($p$-value)
% Specifically, since ba-local does not provide ground truth positions, we directly calculate the RMSE between the original and no-marking LiDAR localization results



==> motivation.tex <==
\nsection{Defense Motivation and Challenges} \label{sec:motivation}

In this section, we first evaluate whether the recent physical-invariant based defenses can effectively detect the existing AD localization attack. Motivated by the limitations of these defenses, we then identify the unique challenges for effective defenses in the high-level AD context.

% \subsection{Detection Effectiveness of Physical-Invariant based Defenses against AD localization Attack}
\nsubsection{Effectiveness of Existing Defenses} \label{sec:motivation_savior}

\textbf{Evaluation methodology.} 
We evaluate the detection effectiveness of physical-invariant based defenses against \fr{}~\cite{fusionripper}, which attacks MSF based AD localization using GPS spoofing. In our evaluation, we focus on SAVIOR~\cite{savior} rather than CI~\cite{ci} since SAVIOR adopts more complex nonlinear state estimation models and has shown superior detection performance than CI~\cite{savior}. Following the similar methodology as in SAVIOR's ground rover evaluation, we use the kinematic bicycle model~\cite{kong2015kinematic} and an Extended Kalman Filter (EKF) to predict the system state (i.e., position in x, y coordinates) given the vehicle control commands (i.e., steering and acceleration). Although the vanilla bicycle model does not have tunable parameters, we follow a similar implementation as SAVIOR by adding coefficients to the bicycle model equations~\cite{savior_code}. Same as SAVIOR, we use the \textit{nlgreyest} system identification tool from Matlab~\cite{matlab_si} to find the coefficients that can best fit the sensor and control trace.

During the evaluation, we continuously calculate the residuals between the GPS measurements and the predicted positions from the EKF, and feed the residuals to a CUSUM anomaly detector for attack detection. An execution that triggers the CUSUM detector will be considered as under attack. Specifically, we calculate the true positive rate (TPR) and false positive rate (FPR) by evaluating SAVIOR on the spoofed GPS traces and benign GPS traces and their corresponding control outputs, respectively. To systematically evaluate the detection performance, we vary the CUSUM thresholds to obtain the Receiver Operating Characteristic (ROC) curve.

\textbf{Experimental setup.}
For illustration purpose, we present the evaluation results on \textit{ka-local31}, which is a local road KAIST trace~\cite{jeong2019complex} (More SAVIOR evaluations will be presented in \S\ref{sec:eval_detection}). Since the KAIST traces do not contain control outputs, we replay the trace in Baidu Apollo to record the vehicle control commands (more details in Appendix~\ref{app:savior_collect_control}). In our evaluation, we use the best GPS spoofing parameters ($d$=0.5 m, $f$=1.2), which can achieve over 99\% success rate for the \textit{off-road} attack on Baidu Apollo MSF~\cite{fusionripper}.

\textbf{SAVIOR detection effectiveness and analysis.}
Fig.~\ref{fig:motivation_savior_roc} shows the ROC curve of SAVIOR on \textit{ka-local31}. As shown, SAVIOR's detection performance is only slightly better than random guessing and far from a perfect detector. For example, when the TPR of SAVIOR is 100\%, the lowest FPR it can achieve is still at 79\%. Such a detection performance would render the detection method unpractical in real world as it would introduce lots of false positives in normal driving.

% The root cause behind the poor detection performance is that \textit{the physical invariants used in the existing defenses, e.g., bicycle model, are not accurate enough to detect stealthy attacks targeting high-level AD systems}, which generally have much more sophisticate system designs and thus have more stringent requirement on attack stealthiness. Due to the inaccuracy of the predicted system state from the physical invariants, the existing defenses have to set a relatively large threshold to tolerate the deviations between the predicted state and the sensor measurement in the benign scenarios. While this might be acceptable for robotics vehicles such as drones and ground rovers, which have less requirement on attack stealthiness, attacks targeting high-level AD systems has to use small attack parameters to prevent being recognized as outliers, e.g., \fr{} on \textit{ka-local31} uses a sub-meter spoofing distance (0.5 m) during its first attack stage. In comparison, the bicycle model used in SAVIOR is reported to have an average position error of 0.33 m within 0.8 sec under low-speed settings (e.g., 13.8 m/s) in~\cite{kong2015kinematic} and its error keeps accumulating as time progresses; comparably, the same bicycle model incurs an average error of 1.076 m on \textit{ka-local31} within 1 sec.

The reason behind the poor detection performance in the AD context is twofold. First, the physical dynamics of the vehicle are much harder to model due to the complex physical moving characteristics, e.g., tire-road frictions, aerodynamic forces, road bank angles, etc.~\cite{rajamani2011vehicle}. For example, prior study~\cite{polack2017kinematic} finds that the error of kinematic bicycle model increases very fast at high speeds (e.g., 25 $\mathrm{m/s}$) or on curvy roads (e.g., steering angle at 4$^\circ$). In comparison, the bicycle model used in SAVIOR is reported having an average position error of 0.33 m \textit{within 0.8 sec} under low-speed settings (e.g., 13.8 m/s) in~\cite{kong2015kinematic} and its error keeps accumulating as time progresses; comparably, the same bicycle model incurs an average error of 1.076 m on \textit{ka-local31} within 1 sec, where the trace contains many turns and curvy roads.

Second, the attack deviation goals in the AD context can be much smaller but still being safety-critical. 
While SAVIOR is effective at detecting attacks on small robotics vehicles such as drones with large deviation goals (e.g., $\sim$50 m~\cite{savior}), attacks targeting high-level AD systems requires much smaller deviation and thus harder to detect. For example, even less than 0.5 m lateral deviations are enough to cause lane departure on narrow urban roads (e.g., 2.7 m wide~\cite{road_shoulder_width}).

\junjie{position against SAVIOR: current savior design is limited, cite bicycle model problem. Then say we explore a different defense direction from SAVIOR. It is not to dismiss the line of work like SAVIOR and CI is not usable.}

% \junjie{I deleted the natural GPS deviation arguement since that is not so fundamental.}

% Due to the inaccuracy of the predicted system state from the physical invariants, the existing defenses have to set a relatively large threshold to tolerate the deviations between the predicted state and the sensor measurement in the benign scenarios. While this might be acceptable for robotics vehicles such as drones and ground rovers, which have less requirement on attack stealthiness, attacks targeting high-level AD systems has to use small attack parameters to prevent being recognized as outliers, e.g., \fr{} on \textit{ka-local31} uses a sub-meter spoofing distance (0.5 m) during its first attack stage. 

\cut{
Another reason for the high FPR in SAVIOR is that \textit{GPS measurements can naturally have large fluctuations} because of the satellite signal inferences during the transmission~\cite{gps_error_sources}, which may trigger false detection if a benign GPS measurement has a large deviation to the ground truth position of the vehicle. To verify this, we calculate the deviations between the benign GPS and the ground truth positions in the KAIST traces. As shown in Fig.~\ref{fig:motivation_gps_devs}, the natural GPS deviations have a long-tail distribution, where majority of the GPS measurements has less than 0.4 m deviation. But still, there exists many measurements with deviations $>$6.5 m, and note that the KAIST dataset uses a high-end GPS receiver (SOKKIA GRX2), which costs around \$8000~\cite{kaist_gps_price}.}

\begin{figure}[tbp]
\centering
\includegraphics[width=.55\linewidth]{./figs/motivation_ka-local31_roc.pdf}
\vspace{-0.15in}
\caption{Detection ROC curve of SAVIOR on a KAIST trace, \textit{ka-local31}, against the \fr{} attack.}
\label{fig:motivation_savior_roc}
\vspace{-0.05in}
\end{figure}

% \begin{figure}[tbp]
% \centering
% \includegraphics[width=.7\linewidth]{./figs/natural_gps_devs.pdf}
% \vspace{-0.1in}
% \caption{Long-tail distribution of natural GPS deviations to the ground truth positions in KAIST traces.}
% \label{fig:motivation_gps_devs}
% \end{figure}

% \begin{table}[tbp]
% \footnotesize
% \begin{minipage}{0.485\linewidth}
% 	\centering
%     \includegraphics[width=\columnwidth]{./figs/motivation_ka-local31_roc.pdf}
%     \vspace{-0.27in}
%     \captionof{figure}{Detection ROC curve of SAVIOR on a \textit{ka-local31} against the \fr{} attack.}
%     \label{fig:motivation_savior_roc}
% \end{minipage}\hfill\hspace{0.015\linewidth}
% \begin{minipage}{0.485\linewidth}
% 	\centering
%     \includegraphics[width=\columnwidth]{./figs/natural_gps_devs.pdf}
%     \vspace{-0.25in}
%     \captionof{figure}{Long-tail distribution of natural GPS deviations to the ground truth positions in KAIST traces.}
%     \label{fig:motivation_gps_devs}
% \end{minipage}
% \vspace{-0.1in}
% \end{table}


